COLD: Causal reasOning in cLosed Daily activities

Large Language Models (LLMs) have shown state-of-the-art performance in a variety of tasks, including arithmetic and reasoning; however, to gauge the intellectual capabilities of LLMs, causal reasoning has become a reliable proxy for validating a general understanding of the mechanics and intricacies of the world similar to humans. Previous works in natural language processing (NLP) have either focused on open-ended causal reasoning via causal commonsense reasoning (CCR) or framed a symbolic representation-based question answering for theoretically backed-up analysis via a causal inference engine. The former adds an advantage of real-world grounding but lacks theoretically backed-up analysis/validation, whereas the latter is far from real-world grounding. In this work, we bridge this gap by proposing the COLD (Causal reasOning in cLosed Daily activities) framework, which is built upon human understanding of daily real-world activities to reason about the causal nature of events. We show that the proposed framework facilitates the creation of enormous causal queries (~ 9 million) and comes close to the mini-turing test, simulating causal reasoning to evaluate the understanding of a daily real-world task. We evaluate multiple LLMs on the created causal queries and find that causal reasoning is challenging even for activities trivial to humans. We further explore (the causal reasoning abilities of LLMs) using the backdoor criterion to determine the causal strength between events.

==> sections/human-validation.tex <==
\section{Human validation}
% To get a rough estimate of the human performance on the created causal reasoning queries, we also perform small-scale human annotations, where the annotators are given a set of randomly chosen 100 causal queries. Table App. \ref{tab:human_performance} shows the obtained results.
% We would like to mention that validating human performance is challenging due to the nature of the causal reasoning task. The nature of counterfactual reasoning requires the human/algorithm to assume a similar alternate world/universe with only a particular happening or not happening to approximate the causal strength between the events. These imaginations can be expressed in statements as highlighted by \cite{bookOfWhy, pearl2016causal}, containing an “if” statement in which the “if” portion is untrue or unrealized (aka counterfactual). The “if” portion of a counterfactual is called the hypothetical condition, or more often, the antecedent, making it challenging (cognitively heavy) to conduct a human evaluation.
% We report the performance on a small sample of 100 causal query triplets (note that the dataset can contain an enormous number of causal queries), and generalizing it as a human performance may not be scientifically correct and could contain some biased estimates of human benchmarking present in the paper (i.e., the presented estimates may not be true representative of the entire population). Hence, we recommend considering these numbers with a grain of salt.

